Decoding Dependency Risks: A Quantitative Study of Vulnerabilities in the Maven Ecosystem

This study investigates vulnerabilities within the Maven ecosystem by analyzing a comprehensive dataset of 14,459,139 releases. Our analysis reveals the most critical weaknesses that pose significant threats to developers and their projects as they look to streamline their development tasks through code reuse. We show risky weaknesses, those unique to Maven, and emphasize those becoming increasingly dangerous over time. Furthermore, we reveal how vulnerabilities subtly propagate, impacting 31.39% of the 635,003 latest releases through direct dependencies and 62.89% through transitive dependencies. Our findings suggest that improper handling of input and mismanagement of resources pose the most risk. Additionally, Insufficient session-ID length in J2EE configuration and no throttling while allocating resources uniquely threaten the Maven ecosystem. We also find that weaknesses related to improper authentication and managing sensitive data without encryption have quickly gained prominence in recent years. These findings emphasize the need for proactive strategies to mitigate security risks in the Maven ecosystem.

==> info/howTo.tex <==
\subsection{Units}
\begin{itemize}
\item Use either SI (MKS) or CGS as primary units. (SI units are encouraged.) English units may be used as secondary units (in parentheses). An exception would be the use of English units as identifiers in trade, such as ``3.5-inch disk drive''.
\item Avoid combining SI and CGS units, such as current in amperes and magnetic field in oersteds. This often leads to confusion because equations do not balance dimensionally. If you must use mixed units, clearly state the units for each quantity that you use in an equation.
\item Do not mix complete spellings and abbreviations of units: ``Wb/m\textsuperscript{2}'' or ``webers per square meter'', not ``webers/m\textsuperscript{2}''. Spell out units when they appear in text: ``. . . a few henries'', not ``. . . a few H''.
\item Use a zero before decimal points: ``0.25'', not ``.25''. Use ``cm\textsuperscript{3}'', not ``cc''.)
\end{itemize}

\begin{table}[htbp]
\caption{Table Type Styles}
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Table}&\multicolumn{3}{|c|}{\textbf{Table Column Head}} \\
\cline{2-4} 
\textbf{Head} & \textbf{\textit{Table column subhead}}& \textbf{\textit{Subhead}}& \textbf{\textit{Subhead}} \\
\hline
copy& More table copy$^{\mathrm{a}}$& &  \\
\hline
\multicolumn{4}{l}{$^{\mathrm{a}}$Sample of a Table footnote.}
\end{tabular}
\label{tab1}
\end{center}
\end{table}

\begin{figure}[htbp]
\centerline{\includegraphics{images/fig1.png}}
\caption{Example of a figure caption.}
\label{fig}
\end{figure}

Figure Labels: Use 8 point Times New Roman for Figure labels. Use words 
rather than symbols or abbreviations when writing Figure axis labels to 
avoid confusing the reader. As an example, write the quantity 
``Magnetization'', or ``Magnetization, M'', not just ``M''. If including 
units in the label, present them within parentheses. Do not label axes only 
with units. In the example, write ``Magnetization (A/m)'' or ``Magnetization 
\{A[m(1)]\}'', not just ``A/m''. Do not label axes with a ratio of 
quantities and units. For example, write ``Temperature (K)'', not 
``Temperature/K''.


\bibitem{b2} J. Clerk Maxwell, A Treatise on Electricity and Magnetism, 3rd ed., vol. 2. Oxford: Clarendon, 1892, pp.68--73.
\bibitem{b3} I. S. Jacobs and C. P. Bean, ``Fine particles, thin films and exchange anisotropy,'' in Magnetism, vol. III, G. T. Rado and H. Suhl, Eds. New York: Academic, 1963, pp. 271--350.
\bibitem{b4} K. Elissa, ``Title of paper if known,'' unpublished.
\bibitem{b5} R. Nicole, ``Title of paper with only first word capitalized,'' J. Name Stand. Abbrev., in press.
\bibitem{b6} Y. Yorozu, M. Hirano, K. Oka, and Y. Tagawa, ``Electron spectroscopy studies on magneto-optical media and plastic substrate interface,'' IEEE Transl. J. Magn. Japan, vol. 2, pp. 740--741, August 1987 [Digests 9th Annual Conf. Magnetics Japan, p. 301, 1982].
\bibitem{b7} M. Young, The Technical Writer's Handbook. Mill Valley, CA: University Science, 1989.
%\end{thebibliography}
\vspace{12pt}
\color{red}
IEEE conference templates contain guidance text for composing and formatting conference papers. Please ensure that all template text is removed from your conference paper prior to submission to the conference. Failure to remove the template text from your paper may result in your paper not being published.


Please number citations consecutively within brackets \cite{b1}. The 
sentence punctuation follows the bracket \cite{b2}. Refer simply to the reference 
number, as in \cite{b3}---do not use ``Ref. \cite{b3}'' or ``reference \cite{b3}'' except at 
the beginning of a sentence: ``Reference \cite{b3} was the first $\ldots$''

Number footnotes separately in superscripts. Place the actual footnote at 
the bottom of the column in which it was cited. Do not put footnotes in the 
abstract or reference list. Use letters for table footnotes.

Unless there are six authors or more give all authors' names; do not use 
``et al.''. Papers that have not been published, even if they have been 
submitted for publication, should be cited as ``unpublished'' \cite{b4}. Papers 
that have been accepted for publication should be cited as ``in press'' \cite{b5}. 
Capitalize only the first word in a paper title, except for proper nouns and 
element symbols.

For papers published in translation journals, please give the English 
citation first, followed by the original foreign-language citation \cite{b6}.



\subsection{\LaTeX-Specific Advice}

Please use ``soft'' (e.g., \verb|\eqref{Eq}|) cross references instead
of ``hard'' references (e.g., \verb|(1)|). That will make it possible
to combine sections, add equations, or change the order of figures or
citations without having to go through the file line by line.

Please don't use the \verb|{eqnarray}| equation environment. Use
\verb|{align}| or \verb|{IEEEeqnarray}| instead. The \verb|{eqnarray}|
environment leaves unsightly spaces around relation symbols.

Please note that the \verb|{subequations}| environment in {\LaTeX}
will increment the main equation counter even when there are no
equation numbers displayed. If you forget that, you might write an
article in which the equation numbers skip from (17) to (20), causing
the copy editors to wonder if you've discovered a new method of
counting.

{\BibTeX} does not work by magic. It doesn't get the bibliographic
data from thin air but from .bib files. If you use {\BibTeX} to produce a
bibliography you must send the .bib files. 

{\LaTeX} can't read your mind. If you assign the same label to a
subsubsection and a table, you might find that Table I has been cross
referenced as Table IV-B3. 

{\LaTeX} does not have precognitive abilities. If you put a
\verb|\label| command before the command that updates the counter it's
supposed to be using, the label will pick up the last counter to be
cross referenced instead. In particular, a \verb|\label| command
should not go before the caption of a figure or a table.

Do not use \verb|\nonumber| inside the \verb|{array}| environment. It
will not stop equation numbers inside \verb|{array}| (there won't be
any anyway) and it might stop a wanted equation number in the
surrounding equation.

\subsection{Some Common Mistakes}\label{SCM}
\begin{itemize}
\item The word ``data'' is plural, not singular.
\item The subscript for the permeability of vacuum $\mu_{0}$, and other common scientific constants, is zero with subscript formatting, not a lowercase letter ``o''.
\item In American English, commas, semicolons, periods, question and exclamation marks are located within quotation marks only when a complete thought or name is cited, such as a title or full quotation. When quotation marks are used, instead of a bold or italic typeface, to highlight a word or phrase, punctuation should appear outside of the quotation marks. A parenthetical phrase or statement at the end of a sentence is punctuated outside of the closing parenthesis (like this). (A parenthetical sentence is punctuated within the parentheses.)
\item A graph within a graph is an ``inset'', not an ``insert''. The word alternatively is preferred to the word ``alternately'' (unless you really mean something that alternates).
\item Do not use the word ``essentially'' to mean ``approximately'' or ``effectively''.
\item In your paper title, if the words ``that uses'' can accurately replace the word ``using'', capitalize the ``u''; if not, keep using lower-cased.
\item Be aware of the different meanings of the homophones ``affect'' and ``effect'', ``complement'' and ``compliment'', ``discreet'' and ``discrete'', ``principal'' and ``principle''.
\item Do not confuse ``imply'' and ``infer''.
\item The prefix ``non'' is not a word; it should be joined to the word it modifies, usually without a hyphen.
\item There is no period after the ``et'' in the Latin abbreviation ``et al.''.
\item The abbreviation ``i.e.'' means ``that is'', and the abbreviation ``e.g.'' means ``for example''.
\end{itemize}
An excellent style manual for science writers is \cite{b7}.

\subsection{Authors and Affiliations}
\textbf{The class file is designed for, but not limited to, six authors.} A 
minimum of one author is required for all conference articles. Author names 
should be listed starting from left to right and then moving down to the 
next line. This is the author sequence that will be used in future citations 
and by indexing services. Names should not be listed in columns nor group by 
affiliation. Please keep your affiliations as succinct as possible (for 
example, do not differentiate among departments of the same organization).

\subsection{Identify the Headings}
Headings, or heads, are organizational devices that guide the reader through 
your paper. There are two types: component heads and text heads.

Component heads identify the different components of your paper and are not 
topically subordinate to each other. Examples include Acknowledgments and 
References and, for these, the correct style to use is ``Heading 5''. Use 
``figure caption'' for your Figure captions, and ``table head'' for your 
table title. Run-in heads, such as ``Abstract'', will require you to apply a 
style (in this case, italic) in addition to the style provided by the drop 
down menu to differentiate the head from the text.

Text heads organize the topics on a relational, hierarchical basis. For 
example, the paper title is the primary text head because all subsequent 
material relates and elaborates on this one topic. If there are two or more 
sub-topics, the next level head (uppercase Roman numerals) should be used 
and, conversely, if there are not at least two sub-topics, then no subheads 
should be introduced.

\subsection{Figures and Tables}
\paragraph{Positioning Figures and Tables} Place figures and tables at the top and 
bottom of columns. Avoid placing them in the middle of columns. Large 
figures and tables may span across both columns. Figure captions should be 
below the figures; table heads should appear above the tables. Insert 
figures and tables after they are cited in the text. Use the abbreviation 
``Fig.~\ref{fig}'', even at the beginning of a sentence.

==> sections/analysis.tex <==

% \input{sections/analysis_cwe}



% \input{sections/analysis_propagation}



==> sections/analysis_cwe.tex <==

\subsection{CWE Analysis}
%\vspace{-11pt}



\subsubsection{Equations}


% \begin{table}[t!]\centering
% \caption{Count of top 33.33\% CWEs}
% \label{table:cwe_summary}
% \begin{tblr}{|@{ }l|r||l|r||l|r@{ }|}
% \hline
% \textbf{CWE} & \textbf{Count} & \textbf{CWE} & \textbf{Count} & \textbf{CWE} & \textbf{Count} \\
% \hline
% CWE-502 & 17187 & CWE-532 & 1806 & CWE-1295 & 778 \\
% CWE-79  & 16426 & CWE-83  & 1691 & CWE-78  & 759 \\
% CWE-400 & 13633 & CWE-203 & 1669 & CWE-276 & 747 \\
% CWE-20  & 11693 & CWE-362 & 1641 & CWE-148 & 716 \\
% CWE-22  & 10352 & CWE-285 & 1476 & CWE-270 & 715 \\
% CWE-200 & 10226 & CWE-522 & 1401 & CWE-401 & 697 \\
% CWE-611 & 6089  & CWE-787 & 1356 & CWE-190 & 620 \\
% CWE-770 & 5356  & CWE-120 & 1238 & CWE-639 & 620 \\
% CWE-94  & 4965  & CWE-613 & 1228 & CWE-116 & 609 \\
% CWE-287 & 4817  & CWE-552 & 1212 & CWE-201 & 594 \\
% CWE-444 & 4221  & CWE-379 & 1207 & CWE-90  & 565 \\
% CWE-863 & 4095  & CWE-384 & 1174 & CWE-306 & 555 \\
% CWE-918 & 3264  & CWE-378 & 1169 & CWE-358 & 550 \\
% CWE-269 & 2951  & CWE-732 & 1099 & CWE-119 & 547 \\
% CWE-668 & 2828  & CWE-345 & 966 & CWE-80  & 536 \\
% CWE-352 & 2765  & CWE-459 & 958 & CWE-338 & 530 \\
% CWE-295 & 2755  & CWE-434 & 952 & CWE-346 & 510 \\
% CWE-601 & 2678  & CWE-674 & 939 & CWE-311 & 444 \\
% CWE-284 & 2641  & CWE-209 & 905  & CWE-95  & 441 \\
% CWE-74  & 2560  & CWE-377 & 904   & CWE-319 & 408 \\
% CWE-835 & 2548  & CWE-281 & 877 & CWE-184 & 403 \\
% CWE-862 & 2131  & CWE-208 & 829 & CWE-290 & 401 \\
% CWE-917 & 2100  & CWE-347 & 870  & CWE-1333 & 398 \\
% CWE-89  & 2064  & CWE-330 & 793 &  CWE-1321 & 391\\
% CWE-755 & 1821  & CWE-77  & 788 &  CWE-789  & 387\\
% \hline
% \end{tblr}
% \end{table}






% \begin{table*}[t!]\centering
% \caption{CWE Categories and Vulnerability Counts (Non-Zero Categories Only)}
% \label{table:cwe_categories_sorted}
% \begin{tblr}{|Q[5cm,valign=m,colsep=5pt]|Q[2cm,valign=m,colsep=5pt]|Q[2cm,valign=m,colsep=5pt]|}
% \hline
% \textbf{Category} & \textbf{CWE Count} & \textbf{Vulnerability Count} \\
% \hline
% API / Function Errors & 7 & 25910 \\
% Data Neutralization Issues & 21 & 15917 \\
% Resource Management Errors & 21 & 9350 \\
% File Handling Issues & 9 & 5838 \\
% Authorization Errors & 9 & 5227 \\
% Behavioral Problems & 18 & 3885 \\
% Business Logic Errors & 8 & 2972 \\
% Data Integrity Issues & 16 & 2381 \\
% Memory Buffer Errors & 9 & 2291 \\
% Data Validation Issues & 12 & 2393 \\
% Information Management Errors & 18 & 2651 \\
% Communication Channel Errors & 13 & 1235 \\
% Concurrency Issues & 11 & 828 \\
% User Interface Security Issues & 9 & 560 \\
% User Session Errors & 3 & 445 \\
% Audit / Logging Errors & 6 & 595 \\
% Authentication Errors & 15 & 1028 \\
% Cryptographic Issues & 12 & 347 \\
% Key Management Errors & 4 & 347 \\
% Numeric Errors & 9 & 193 \\
% Pointer Issues & 10 & 514 \\
% Privilege Issues & 13 & 281 \\
% Permission Issues & 10 & 281 \\
% Initialization and Cleanup Errors & 8 & 459 \\
% \hline
% \end{tblr}
% \end{table*}



% \begin{table*}[ht]
% \centering
% \caption{Counts of CWE Entries and Vulnerabilities by Pillar}
% \begin{tabular}{|p{0.35\textwidth}|p{0.15\textwidth}|p{0.20\textwidth}|}
% \hline
% \textbf{Pillar} & \textbf{CWE Count} & \textbf{Vulnerability Count} \\
% \hline
% Improper Neutralization & 51 & 25,833 \\
% Protection Mechanism Failure & 22 & 12,304 \\
% Improper Access Control & 36 & 14,537 \\
% Improper Adherence to Coding Standards & 33 & 8,215 \\
% Improper Control of a Resource Through its Lifetime & 17 & 3,960 \\
% Incorrect Calculation & 10 & 3,075 \\
% Insufficient Control Flow Management & 11 & 2,436 \\
% Improper Interaction Between Multiple Correctly-Behaving Entities & 5 & 1,882 \\
% \hline
% \end{tabular}
% \label{table:pillar_counts}
% \end{table*}

==> sections/analysis_propagation.tex <==
\subsection{RQ4 Analysis}

The findings of our analysis, summarized in Table~\ref{tab:impact_analysis_results}, reveal a striking contrast in the extent to which direct and transitive vulnerabilities impact the latest releases of the Maven ecosystem. These results provide valuable insights into the latent nature of modern dependency networks and highlight the critical need for proactive security measures.

\subsubsection*{Direct Vulnerabilities: A Manageable Frontier?}

Approximately 31.24\% of the latest releases were directly impacted by vulnerabilities. Despite this proportion being significant, it represents a manageable boundary where intervention is feasible. Direct vulnerabilities are, by nature, tied to the immediate dependencies of a release, making them easier to identify and mitigate. This result emphasizes the importance of ensuring security practices at a release level are maintained. This process should include a process of thoroughly vetting dependencies and using automated vulnerability detection tools. Addressing the direct vulnerabilities at the source has great promise to significantly reduce the attack surface for releases.

\subsubsection*{Transitive Vulnerabilities: The Hidden Threat}

A very alarming result from our study is the overwhelming 62.87\% of the latest release being affected by vulnerabilities propagated through three levels of transitive dependencies. To understand the impact of the levels of transitivity, we also explored limiting the analysis to two levels of dependency chains and observed that the proportion of releases impacted drops to 60.14\% accounting for an insignificant difference only a minor 2.73\%.  This finding shows the systemic risks that are posed by indirect dependencies which in essence often form most of the dependency tree artifacts. As opposed to direct vulnerabilities, transitive vulnerabilities are much more challenging to trace and mitigate because they span multiple layers of cascading relationships. Some of these vulnerabilities may originate from rarely updated perhaps even unmaintained dependencies deep in the dependency graph. The nature of these deeply hidden risks magnifies the impact of a single vulnerability which may affect several artifacts. Our finding underscores the scale of this transitive impact demonstrating not only how interconnected and fragile the ecosystem is but also the critical need for tools that would provide developers with deeper insights into risks that are hiding in plain sight.

\subsubsection*{Implications for Ecosystem Security}
Our results reveal that transitive vulnerabilities represent a more prevalent and challenging problem than direct vulnerabilities.  This distinction calls for a paradigm shift in how developers and ecosystem maintainers approach the essential task of dependency management. Traditional practices that focus only on direct dependencies not sufficient in effectively mitigating risks that are propagated through the transitive chain. To minimize the impact of the uncovered vulnerabilities, we propose:
Ecosystem tools should consider integrating deeper insights into transitive dependencies with the goal of offering proactive alerts and recommendations to developers.
Further, collaborative efforts among library maintainers should be fostered such as safely deprecating unmaintained dependencies and enforcing much more strict security checks for widely used artifacts to reduce the risk of transitive vulnerabilities. Furthermore, incorporating automated updates for vulnerable dependencies is another avenue of exploration especially for transitive ones as this would significantly improve the security posture of the entire ecosystem. Our replication package~\cite{b1} provides the specific vulnerabilities at different levels of transitivity for the latest releases that may be a starting point before extending to the entire ecosystem.



\input{illustrations/RQ4_table}

==> sections/result.tex <==
\subsubsection{RQ1} 
% How has the number of vulnerable releases changed over the years?
\input{sections/rq1}

% \section{RQ2: What kind of weaknesses are prevalent in the ecosystem?

\subsubsection{RQ2}
% What types of weaknesses are most dangerous in the ecosystem? How do weaknesses in Maven differ from the formal list?
\input{sections/rq2}


\subsubsection{RQ3}
 % Which weaknesses are gaining momentum?
\input{sections/rq3}

\subsubsection{RQ4}
% What proportion of releases are impacted directly and transitively?
\input{sections/rq4}
